Manipulating Highly Deformable Materials Using a Visual Feedback Dictionary

The complex physical properties of highly deformable materials such as clothes pose significant challenges fanipulation systems. We present a novel visual feedback dictionary-based method for manipulating defoor autonomous robotic mrmable objects towards a desired configuration. Our approach is based on visual servoing and we use an efficient technique to extract key features from the RGB sensor stream in the form of a histogram of deformable model features. These histogram features serve as high-level representations of the state of the deformable material. Next, we collect manipulation data and use a visual feedback dictionary that maps the velocity in the high-dimensional feature space to the velocity of the robotic end-effectors for manipulation. We have evaluated our approach on a set of complex manipulation tasks and human-robot manipulation tasks on different cloth pieces with varying material characteristics.

==> archive/vs.tex <==
\section{Visual Servoing}
In this section, we will follow the notation and concepts defined in \cite{bateux2017histograms} \cite{bateux2015direct}. For the original setup of their task is a positioning problem and ours is a manipulation of the deformable objects. 

\subsection{Theoretical Foundation}
The aim of the manipulation task for the deformable body is to reach a desired state $t*$, where the configuration of the end-effectors is $r^*$, starting from an arbitrary initial configuration $r_0$, which is quite similar to the positioning task described in \cite{bateux2017histograms}.
To achieve the goal, we needs to define both representation which indicate the state of $t$ and the cost function which reflects the difference between two different configuration $r$ and $r'$. Considering the actual position of end-effectors of the deformable object as $r$, the problem can be formulated as an optimization process:
\begin{equation}
\hat{r} = \underset{r}{\operatorname{argmax}} \rho(r, r^*)
\end{equation}

where $\rho(.)$ is the error function between the two different configuration of the deformable objects. If the we assume the uniqueness of $t$ for each corresponding $r$, we can transfer the cost function into a map from $t$. 

\begin{equation}
\hat{r} = \underset{r}{\operatorname{argmax}} \rho'(t, t^*)
\end{equation}
where $\rho'(.)$ is the error function between the two different states of the deformable objects. And the closest solution to the function will be $\hat{r}$. 
Considering the feature space $s$, the task is can be formulated as finding a closest solution between $s^*$ and $s(r)$:
\begin{equation}
\hat{s} = \underset{r}{\operatorname{argmax}} \rho''(s(r), s(r^*))
\end{equation}

where $\rho''(.)$ is the error function mapping from the feature space.  For the visual servoing task can be achieved by applying a velocity $v$ to the end effectors of the deformable objects, which links from the variation of the feature. 
\begin{equation}
v = -\lambda L (s(r) - s^*)
\end{equation}
Where $L$ is a function from the feature space to the controlling parameters. And the $\lambda$ is a positive scalar gain defining the convergence speed. 


\subsection{Histogram-Based Visual Servoing}
A histogram is an approximation of the distribution of a variable, which can be used to  reduce the redundancy of data and extract the higher level of information. It induces more robustness to the local variation. And for some histogram like HOG \cite{dalal2005histograms}, it reduces the dependency of the illumination conditions and avoid the pixel-level comparison. 

In the setup of the positioning task described in \cite{bateux2017histograms},  it follows the definition of the interaction matrix $L$ in \cite{chaumette2006visual}. 
\begin{equation}
L = \frac{\partial s}{\partial r}
\end{equation}
When $s$ is the feature of the image in the camera position $r$, $L$ can be represented by 
\begin{equation}
L = \frac{\partial \rho(s, s*) }{\partial r}
\end{equation}

However, in our setup,  $r$ is the state of the deformable objects which is a hidden variable which only related with the controlling parameter $c$. 

So we model the map from the $r$ to $s$ as a function $f$ instead of a matrix with parameters as:
\begin{equation}
c - c^* = L(s - s^*)
\end{equation}
And in order to estimate $L$, we apply the sparse linear regression method described in section \ref{sec:regress}.



And $L^+_s$ is the pseudo-inverse of the interaction matrix. They use the Levenberg-Marquardt(LM) optimization approach to solve the controlling laws, see details in \cite{collewet2011photometric}:
%\begin{equation}
%v = -\lambda(H_I + \mu \textbf{diag}(H_I))^{-1} L_I^T (I-I^*)
%\end{equation}
%Where $H_I = L^T_I L_I$

\subsubsection{Histogram-based Visual Servoing}
A histogram-based feature is an approximation to the raw image, which can reduce the data redundancy and can extract a high-level representation that is robust to local variation in an image. Histogram-based features have been adopted by~\cite{bateux2017histograms, bateux2015direct}
to achieve a general framework for photometric visual servoing. In addition, they modify the definition of the  interaction matrix from $L_H = \frac{\partial s_H}{\partial r}$ to 
\begin{equation}
\label{eq:l_h}
L_H = \frac{\partial \rho(s_H, s_H^*) }{\partial r},
\end{equation}
where the subscript $H$ indicates the histogram feature and $L_H$ is also computed using Levenberg-Marquardt optimization. Then the control law can be formulated as
\begin{equation}
\label{eq:velocity}
v = -\lambda L^+_H \rho(s_H, s_H^*).
\end{equation}

%By definition, they modify the interaction matrix from the equation \ref{eq:l_s} which equals $L = \frac{\partial s_H}{\partial r}$ to:
%\begin{equation}
%\label{eq:l_h}
%L_H = \frac{\partial \rho(s_H, s_H*) }{\partial r}
%\end{equation}
%They substitute the error in feature space to a cost function $\rho (.)$. After apply a non-linear minimization like Levenberg-Marquardt, the controlling law of HBVS can be formed as:
%\begin{equation}
%v = -\lambda(H_H + \mu \textbf{diag}(H_H))^{-1} L_H^T \rho %(s_H,s_H^*)
%\end{equation}
%where $H_H = L^T_H L_H$.



==> header.tex <==
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{prettyref}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{xcolor}
\usepackage{subfig}
\usepackage{MnSymbol}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{bm}

%\usepackage{enumitem}
%\usepackage{mathtools}
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) #1}
\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}
% Syntax: \colorboxed[<color model>]{<color specification>}{<math formula>}
\newcommand*{\colorboxed}{}
\def\colorboxed#1#{%
  \colorboxedAux{#1}%
}
\newcommand*{\colorboxedAux}[3]{%
  % #1: optional argument for color model
  % #2: color specification
  % #3: formula
  \begingroup
    \colorlet{cb@saved}{.}%
    \color#1{#2}%
    \boxed{%
      \color{cb@saved}%
      #3%
    }%
  \endgroup
}
% ------------------------------------------------------------------------

% ------------------------------------------------------------------------equation
\newrefformat{Fig}{Figure~\ref{#1}}
\newrefformat{fig}{Figure~\ref{#1}}
\newrefformat{par}{Section~\ref{#1}}
\newrefformat{appen}{Appendix~\ref{#1}}
\newrefformat{sec}{Section~\ref{#1}}
\newrefformat{sub}{Section~\ref{#1}}
%\newrefformat{table}{Table~\ref{#1}}
\newrefformat{alg}{Algorithm~\ref{#1}}
\newrefformat{Alg}{Algorithm~\ref{#1}}
\newrefformat{Def}{Definition~\ref{#1}}
\newrefformat{Thm}{Theorem~\ref{#1}}
\newrefformat{step}{Step~\ref{#1}}
\newrefformat{ln}{Line~\ref{#1}}
\newrefformat{eq}{Equation~\ref{#1}}
\newrefformat{pb}{Problem~\ref{#1}}
\newrefformat{it}{Item~\ref{#1}}
\newrefformat{te}{Term~\ref{#1}}
\def\Eqref Eq:#1:{\eqref{eq:#1}}
\newrefformat{Eq}{Equation~\Eqref#1:}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\shortref}[2]{Fig.\ref{#1}#2}
\newcommand{\CTR}{\textbf{:}}
\newcommand{\IDD}{\operatorname{Id}}
\newcommand{\COMP}{\mathcal{O}}
\newcommand{\T}[1]{\tilde{#1}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\TODO}[1]{\textcolor{red}{#1}}
\newcommand{\E}[1]{\mathbf{#1}}
\newcommand{\TE}[1]{\textbf{#1}}
\newcommand{\B}[1]{\boldsymbol{#1}}
%\newcommand{\FPPAT}[3]{\frac{\partial{#1}}{\partial{#2}}\Bigr|_{#3}}
\newcommand{\FPPAT}[3]{\frac{\partial{#1}}{\partial{#3}}}
\newcommand{\FPP}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\FPPT}[2]{\frac{\partial^2{#1}}{\partial{#2}^2}}
\newcommand{\FPPTTT}[2]{\frac{\partial^3{#1}}{\partial{#2}^3}}
\newcommand{\FPPTT}[3]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}}
\newcommand{\FPPM}[3]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}}
\newcommand{\FDD}[2]{\frac{d{#1}}{d{#2}}}
%\newcommand{\FDDR}[2]{{d{#1}}/{d{#2}}}
\newcommand{\FDM}[2]{\frac{D{#1}}{D{#2}}}
\newcommand{\TWO}[2]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{cc}{#1} & {#2}\end{array}\right)}
\newcommand{\TWOC}[2]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{c}#1 \\ #2\end{array}\right)}
\newcommand{\TWOR}[2]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{cc}{#1}^T & {#2}^T\end{array}\right)^T}
\newcommand{\THREE}[3]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{ccc}{#1} & {#2} & {#3}\end{array}\right)}
\newcommand{\THREENB}[3]{\setlength{\arraycolsep}{1pt}\begin{array}{ccc}{#1} & {#2} & {#3}\end{array}}
\newcommand{\THREEC}[3]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{c}#1 \\ #2 \\ #3\end{array}\right)}
\newcommand{\THREER}[3]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{ccc}{#1}^T & {#2}^T & {#3}^T\end{array}\right)^T}
\newcommand{\FOUR}[4]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{cccc}{#1} & {#2} & {#3} & {#4}\end{array}\right)}
\newcommand{\FOURC}[4]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{c}#1 \\ #2 \\ #3 \\ #4\end{array}\right)}
\newcommand{\FOURR}[4]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{cccc}{#1}^T & {#2}^T & {#3}^T & {#4}^T\end{array}\right)^T}
\newcommand{\FIVE}[5]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{ccccc}{#1} & {#2} & {#3} & {#4} & {#5}\end{array}\right)}
\newcommand{\FIVEC}[5]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{c}#1 \\ #2 \\ #3 \\ #4 \\ #5\end{array}\right)}
\newcommand{\FIVER}[5]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{ccccc}{#1}^T & {#2}^T & {#3}^T & {#4}^T & {#5}^T\end{array}\right)^T}
\newcommand{\SIX}[6]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{cccccc}{#1} & {#2} & {#3} & {#4} & {#5} & {#6}\end{array}\right)}
\newcommand{\SIXC}[6]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{c}#1 \\ #2 \\ #3 \\ #4 \\ #5 \\ #6\end{array}\right)}
\newcommand{\SIXR}[6]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{cccccc}{#1}^T & {#2}^T & {#3}^T & {#4}^T & {#5}^T & {#6}^T\end{array}\right)^T}
\newcommand{\MTT}[4]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{cc}#1 & #2 \\ #3 & #4\end{array}\right)}
\newcommand{\MTTF}[9]{\left(\setlength{\arraycolsep}{1pt}
\begin{array}{ccccc}
#1 & #2 & #3 & #4 & #5\\
#6 & & & &\\
#7 & & & &\\
#8 & & & &\\
#9 & & & &
\end{array}\right)}
\newcommand{\MTTT}[9]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{ccc}#1 & #2 & #3 \\ #4 & #5 & #6 \\ #7 & #8 & #9\end{array}\right)}
\newcommand{\MDD}[3]{\left(\setlength{\arraycolsep}{1pt}\begin{array}{ccc}#1 & & \\ & #2 & \\ & & #3\end{array}\right)}
\newcommand{\QUES}[2]{\textcolor{red}{\textit{#1}}--\textcolor{blue}{\textbf{#2}}}
\newcommand{\tr}[1]{\E{tr}(#1)}
\newenvironment{eqntiny}{\begin{tiny}\begin{eqnarray*}}{\end{eqnarray*}\end{tiny}}
\newenvironment{eqntinyN}{\begin{tiny}\begin{eqnarray}}{\end{eqnarray}\end{tiny}}
\newcommand{\fmin}[1]{\underset{#1}{\E{min}}}
\newcommand{\fmax}[1]{\underset{#1}{\E{max}}}
\newcommand{\argmin}[1]{\underset{#1}{\E{argmin}}}
\newcommand{\argminP}[1]{\E{argmin}}
\newcommand{\verteq}{\rotatebox{-90}{$\triangleq$}}
\newcommand{\definedAs}[2]{\underset{\scriptstyle\overset{\mkern4mu\verteq}{#2}}{\underline{#1}}}
%\newcommand{\C}[1]{\left[{#1}\right]_\times}
\newcommand{\TWORCell}[2]{\begin{tabular}{@{}l@{}}#1 \\ #2\end{tabular}}
\newcommand{\THREERCell}[3]{\begin{tabular}{@{}l@{}}#1 \\ #2 \\ #3\end{tabular}}
% ------------------------------------------------------------------------

% ------------------------------------------------------------------------robotics
\newcommand{\LIEG}{SE(3)}
\newcommand{\LIEA}{\mathfrak{se}(3)}
\newcommand{\JR}{{J_\omega}}
\newcommand{\JV}{{J_v}}
\newcommand{\DIAG}{\text{bdiag}}
\newcommand{\KINE}{\mathcal{K}}
\newcommand{\LAG}{\mathcal{L}}
\newcommand{\POT}{\mathcal{P}}
\newcommand{\CROSS}[1]{\left[ #1 \right]}
\newcommand{\CONST}{\text{const.}}
\definecolor{darkgreen}{RGB}{34,172,56}
% ------------------------------------------------------------------------

% ------------------------------------------------------------------------comments
\newcommand{\EMPH}[1]{\textcolor{red}{#1}}
\newcommand{\EMPHB}[1]{\textcolor{blue}{#1}}
\newcommand{\proofread}[1]{\ifProofRead\textcolor{blue}{#1}\fi}
\newenvironment{proofreadBlk}{\color{blue}}{}
\newif\ifProofRead
\ProofReadfalse
% ------------------------------------------------------------------------

